A Systematic Method for Optimum Biomedical Wireless Power Transfer using Inductive Links in Area-Constrained Implants

In the context of implantable bioelectronics, this work provides new insights into maximizing biomedical wireless power transfer (BWPT) via the systematic development of inductive links. This approach addresses the specific challenges of power transfer efficiency (PTE) optimization within the area constraints of bio-implants embedded in tissue. Key contributions include the derivation of an optimal self-inductance with S-parameter-based analyses leading to the co-design of planar spiral coils and L-section impedance matching networks. To validate the proposed design methodology, two coil prototypes -- one symmetric (type-1) and one asymmetric (type-2) -- were fabricated and tested for PTE in pork tissue. Targeting a 20 MHz design frequency, the type-1 coil demonstrated a state-of-the-art PTE of $\sim$ 4\% (channel length = 15 mm) with a return loss (RL) $>$ 20 dB on both the input and output sides, within an area constraint of $<$ 18 $ \times $ 18 mm$^{2}$. In contrast, the type-2 coil achieved a PTE of $\sim$ 2\% with an RL $>$ 15 dB, for a smaller receiving coil area of $<$ 5x5 mm$^{2}$ for the same tissue environment. To complement the coils, we demonstrate a 65 nm test chip with an integrated energy harvester, which includes \asif{a} 30-stage rectifier and low-dropout regulator (LDO), producing a stable $\sim$ 1V DC output within tissue medium, matching theoretical predictions and simulations. Furthermore, we provide a robust and comprehensive guideline for advancing efficient inductive links for various BWPT applications, with shared resources in GitHub available for utilization by the broader community.

==> Author_Bios/Biography.tex <==
\newpage
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{IEEEtran/Author_Bios/Author_AIO.jpg}}]
{Asif Iftekhar Omi}
(S`23) was born in Dhaka, Bangladesh. He received his B.Sc. (Hons.) in Electrical and Electronic Engineering from the Bangladesh University of Engineering and Technology (BUET) in 2014 and completed his M.S. at Washington State University (WSU), USA, in 2022. He is currently pursuing his Ph.D. in Electrical and Computer Engineering at the University of Florida, USA. 

He started his career as a Lecturer at Bangladesh University of Business and Technology (2014-2015), then transitioned to industry roles as a System Engineer at Grameenphone Ltd. and later as a Sub-Divisional Engineer at Dhaka Power Distribution Company Ltd. (2015-2020). In 2021, he joined WSU as a Teaching Assistant (2021-2022), and since 2023, he has been a Graduate Research Assistant at the WISE Lab, University of Florida. His current research interest includes developing energy-efficient Analog/RF/Biomedical integrated circuits and systems for implantable/wearable applications. He was a recipient of the IEEE EMBC NextGen Scholar Award in 2024. 
\end{IEEEbiography}

\vspace{-5mm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{IEEEtran/Author_Bios/Author_AJ.jpg}}]
{Anyu Jiang}
(S`23) received his B.Eng. degree in Information Engineering from the University of Electronic Science and Technology of China (UESTC), Chengdu, China in 2022. He joined the University of Florida in 2023 to pursue his Ph.D. in Electrical and Computer Engineering.
His research interests includes Energy-efficient Analog/Digital circuit design, and Internet of Bodies (IoB). He was a recipient of the IEEE EMBC NextGen Scholar Award in 2024, and a recipient of the IEEE ISSCC SRP and Travel Awards in 2025.
\end{IEEEbiography}

\vspace{-5mm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Author_Bios/Author_BC.png}}]
{Baibhab Chatterjee}
 (M`22) received his Ph.D. from the Elmore Family School of Electrical Engineering, Purdue University, West Lafayette, IN, USA in 2022. He is currently an Assistant Professor in the department of ECE, University of Florida, Gainesville, FL, USA. His industry experience includes two years as a Digital Design Engineer/Senior Digital Design Engineer with Intel, Bengaluru, India, and one year as a Research and Development Engineer with Tejas Networks, Bengaluru, India. He was in the Quantum Hardware Design team with IBM T.J. Watson Research Center, NY, USA during 2020-2021, where he worked on ultra-low power quantum receiver front-ends.
 
 Dr. Chatterjee received the University Gold Medal from NIT Durgapur in 2011, the Institute Silver Medal from IIT Bombay in 2015, the Andrews and Bilsland Fellowships at Purdue University during 2017-2019 and 2021-2022, the HOST 2018 Best Student Poster Award (3rd), the CICC 2019 Best Paper Award (overall), the RFIC/IMS 2020 3MT Award (audience choice) and the Eaton Award in Design Excellence in 2023. His research interests include low-power analog, RF, and mixed-signal circuit design for next-generation biomedical and military applications.
\end{IEEEbiography}
